Online Deep Reinforcement Learning for Autonomous UAV Navigation and Exploration of Outdoor Environments

With the rapidly growing expansion in the use of UAVs, the ability to autonomously navigate in varying environments and weather conditions remains a highly desirable but as-of-yet unsolved challenge. In this work, we use Deep Reinforcement Learning to continuously improve the learning and understanding of a UAV agent while exploring a partially observable environment, which simulates the challenges faced in a real-life scenario. Our innovative approach uses a double state-input strategy that combines the acquired knowledge from the raw image and a map containing positional information. This positional data aids the network understanding of where the UAV has been and how far it is from the target position, while the feature map from the current scene highlights cluttered areas that are to be avoided. Our approach is extensively tested using variants of Deep Q-Network adapted to cope with double state input data. Further, we demonstrate that by altering the reward and the Q-value function, the agent is capable of consistently outperforming the adapted Deep Q-Network, Double Deep Q- Network and Deep Recurrent Q-Network. Our results demonstrate that our proposed Extended Double Deep Q-Network (EDDQN) approach is capable of navigating through multiple unseen environments and under severe weather conditions.

==> old_content.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%old content

Tests were performed using gayscale and RGB images.
\subsection{Autonomous Navigation}

\subsection{Single target: evaluating models}
In this subsection we test the performance of different models through multiple runs. The goal is to define the best model to perform further experiments. All tests were carried using the computer vision module from AirSim. Further tests will be carried using the Drone module from Airsim.

\begin{table}[h]
\centering
\begin{tabular}{@{}llll@{}}
\toprule
Run & \begin{tabular}[c]{@{}l@{}}Total\\ Steps\end{tabular} & \begin{tabular}[c]{@{}l@{}}Predicted\\ Steps\end{tabular} & \begin{tabular}[c]{@{}l@{}}Greedy\\ Steps\end{tabular} \\ \midrule
 1 & 28 & 6 & 22 \\
 2 & 28 & 6 & 22 \\
 3 & 28 & 6 & 22 \\
 4 & 28 & 6 & 22 \\
\bottomrule
\end{tabular}
\caption{Grid 10x10 with memory size of 100 items | target (6,8)}
\label{tab:20x20_100}
\end{table}


\begin{table}[h]
\centering
\begin{tabular}{@{}llll@{}}
\toprule
Run & \begin{tabular}[c]{@{}l@{}}Total\\ Steps\end{tabular} & \begin{tabular}[c]{@{}l@{}}Predicted\\ Steps\end{tabular} & \begin{tabular}[c]{@{}l@{}}Greedy\\ Steps\end{tabular} \\ \midrule
 1 & 150 & 69 & 81 \\
 2 & 150 & 69 & 81 \\
 3 & 150 & 69 & 81 \\
 4 & 150 & 69 & 81 \\
\bottomrule
\end{tabular}
\caption{Grid 20x20 with memory size of 100 items | target (6,18)}
\label{tab:20x20_100}
\end{table}


\begin{table}[h]
\centering
\begin{tabular}{@{}llll@{}}
\toprule
Run & \begin{tabular}[c]{@{}l@{}}Total\\ Steps\end{tabular} & \begin{tabular}[c]{@{}l@{}}Predicted\\ Steps\end{tabular} & \begin{tabular}[c]{@{}l@{}}Greedy\\ Steps\end{tabular} \\ \midrule
 1 & 38 & 6 & 32 \\
 2 & 38 & 6 & 32 \\
 3 & 38 & 6 & 32 \\
 4 & 38 & 6 & 32 \\ \bottomrule
\end{tabular}
\caption{Grid 20x20 with memory size of 400 items | target (6,18)}
\label{tab:20x20_400}
\end{table}


\begin{table}[h]
\centering
\begin{tabular}{@{}llll@{}}
\toprule
Run & \begin{tabular}[c]{@{}l@{}}Total\\ Steps\end{tabular} & \begin{tabular}[c]{@{}l@{}}Predicted\\ Steps\end{tabular} & \begin{tabular}[c]{@{}l@{}}Greedy\\ Steps\end{tabular} \\ \midrule
 \textbf{1} & \textbf{26} & \textbf{19} & \textbf{7} \\
 2 & 150 & 69 & 81 \\
 \textbf{3} & \textbf{26} & \textbf{19} & \textbf{7} \\
 4 & 150 & 69 & 81 \\
 \bottomrule
\end{tabular}
\caption{Grid 20x20 with memory size of 3200 items | target (6,18)}
\label{tab:20x20_3200}
\end{table}

\begin{table}[h]
\centering
\begin{tabular}{@{}llll@{}}
\toprule
Run & \begin{tabular}[c]{@{}l@{}}Total\\ Steps\end{tabular} & \begin{tabular}[c]{@{}l@{}}Predicted\\ Steps\end{tabular} & \begin{tabular}[c]{@{}l@{}}Greedy\\ Steps\end{tabular} \\ \midrule
 1 & 26 & 20 & 6 \\
 2 & 26 & 19 & 7 \\
 3 & 26 & 19 & 7 \\
 4 & 150 & 69 & 81 \\
 5 & 26 & 19 & 7 \\
 6 & 26 & 19 & 7 \\
 7 & 26 & 19 & 7 \\
 8 & 150 & 69 & 81 \\
 9 & 26 & 19 & 7 \\
 10 & 26 & 19 & 7 \\
 \bottomrule
\end{tabular}
\caption{Grid 20x20 with memory size of 3200 items. This code had a bug, which causes the map to start from random positions, but the drone starts from the (0,0) | target (6,18) | reward modified (see reward function)}
\label{tab:20x20_3200_full_reward}
\end{table}

%loading weights from file: ./model_20x20/model_qmaze.h5
As observed on Table \ref{tab:20x20_3200_full_reward} by not normalising the reward values in the range [-1,1], we can reach the target in fewer steps. However, over multiple iterations it sometimes outputs a non-optimal path. Further exploration in the code, allowed the dection of a bug which resulted in the drone being correctly represented in the map with varing starting position, but the AirSim camera being always wrongly initialised from coordinates (0,0,0).
Since, even with this bug the code were capable of outputting the optimal path in the majority of the runs; it makes me think that in reality the algorithm learns quicker if starting always from the same position. The trade off here is, wherever the model will be able to predict optimal paths when not starting the flight from coordinates (0,0,0).


\begin{table}[h]
\centering
\begin{tabular}{@{}llll@{}}
\toprule
Run & \begin{tabular}[c]{@{}l@{}}Total\\ Steps\end{tabular} & \begin{tabular}[c]{@{}l@{}}Predicted\\ Steps\end{tabular} & \begin{tabular}[c]{@{}l@{}}Greedy\\ Steps\end{tabular} \\ \midrule
 1 & 46 & 23 & 23 \\
 2 & 62 & 39 & 23 \\
 3 & 48 & 25 & 23 \\
 4 & 26 & 19 & 7 \\
 5 & 62 & 39 & 23 \\
 6 & 54 & 31 & 23 \\
 7 & 46 & 23 & 23 \\
 8 & 48 & 25 & 23 \\
 9 & 48 & 25 & 23 \\
 10 & 48 & 25 & 23 \\
 \bottomrule
\end{tabular}
\caption{Grid 20x20 with memory size of 3200 items. This code had a bug, which causes the map to start from random positions, but the drone starts from the (0,0) | target (6,18) | reward modified (see reward function)}
\label{tab:20x20_3200_normalised_img_relu}
\end{table}

We now test the relevance of drop out and the learning rate to the network. For this set of results (Table \ref{tab:20x20_3200_normalised_img_drop}) we removed the second drop out and increased the first drop out from 0.2 to 0.5. We also changed reduced the learning rate from 1e-04 to 1e-02.

\begin{table}[h]
\centering
\begin{tabular}{@{}llll@{}}
\toprule
Run & \begin{tabular}[c]{@{}l@{}}Total\\ Steps\end{tabular} & \begin{tabular}[c]{@{}l@{}}Predicted\\ Steps\end{tabular} & \begin{tabular}[c]{@{}l@{}}Greedy\\ Steps\end{tabular} \\ \midrule
 1 & 26 & 19 & 7 \\
 2 & 26 & 19 & 7 \\
 3 & 26 & 19 & 7 \\
 4 & 26 & 19 & 7 \\
 5 & 26 & 19 & 7 \\
 6 & 26 & 19 & 7 \\
 7 & 26 & 19 & 7 \\
 8 & 26 & 19 & 7 \\
 9 & 26 & 19 & 7 \\
 10 & 26 & 19 & 7 \\
 \bottomrule
\end{tabular}
\caption{Grid 20x20 with memory size of 3200 items. This code had a bug, which causes the map to start from random positions, but the drone starts from the (0,0) | target (6,18) }
\label{tab:20x20_3200_normalised_img_drop}
\end{table}

As demonstrated in Table \ref{tab:20x20_3200_normalised_img_drop} the model is capable of outputting the optimal path and maintain consistence over multiple flights. The next set of tests evaluate the ability of the model to learning without the guidance of the greedy approach. We also compare the training time required for each approach.

%20x20_3200_normalised_img_drop/file qmaze_drone_6_paper_0: n_epoch: 334, max_mem: 3200, data: 64, time: 3.58 hours


%%%% The following code is to be used as base to write pseudo-code and/or equations.

\begin{lstlisting}[language=Python, linewidth=\columnwidth,breaklines=true, caption=Reward function]

def get_reward(self):
        drone_row, drone_col, mode = self.state
        pos = [drone_row,drone_col]
        dist = (int(np.linalg.norm(pos-np.array(self.goal))))*(-1)
        
        if drone_row ==self.goal[0] and drone_col == self.goal[1]:
                    return (1.0)
                if mode == 'blocked':
                    return (self.min_reward+dist) - 1
                if (drone_row, drone_col) in self.visited:
                    return (-25+dist)
                if mode == 'invalid':
                    return (-75+dist)
                if mode == 'valid':
                    #return (-4+dist)
                    return (dist)
                    
\end{lstlisting}


The next set of test, trains the network for longer in order to verify if the the network is capable of maintaining consistency over multiple iterations.

\begin{table}[h]
\centering
\begin{tabular}{@{}llll@{}}
\toprule
Run & \begin{tabular}[c]{@{}l@{}}Total\\ Steps\end{tabular} & \begin{tabular}[c]{@{}l@{}}Predicted\\ Steps\end{tabular} & \begin{tabular}[c]{@{}l@{}}Greedy\\ Steps\end{tabular} \\ \midrule
 1 & 120 & 48 & 72 \\
 2 & 150 & 69 & 81 \\
 3 & 38 & 6 & 32 \\
 4 & 26 & 19 & 7 \\
 5 & 120 & 48 & 72 \\
 6 & 38 & 6 & 32 \\
 7 & 120 & 48 & 72 \\
 8 & 150 & 69 & 81 \\
 9 & 120 & 48 & 72 \\
 10 & 38 & 6 & 32 \\
 \bottomrule
\end{tabular}
\caption{Grid 20x20 with memory size of 3200 items, increased win count from 200 to 800| target (6,18)}
\label{tab:20x20_3200_800}
\end{table}

As observed from table \ref{tab:20x20_3200_800} increasing the win count to $2n^2$ does not improve the predictions.

\begin{table}[h]
\centering
\begin{tabular}{@{}llll@{}}
\toprule
Run & \begin{tabular}[c]{@{}l@{}}Total\\ Steps\end{tabular} & \begin{tabular}[c]{@{}l@{}}Predicted\\ Steps\end{tabular} & \begin{tabular}[c]{@{}l@{}}Greedy\\ Steps\end{tabular} \\ \midrule
 1 & 150 & 69 & 81 \\
 2 & 150 & 69 & 81 \\
 3 & 150 & 69 & 81 \\
 4 & 150 & 69 & 81 \\
 \bottomrule
\end{tabular}
\caption{Grid 20x20 with memory size of 3200 items | target (6,18) | reward normalised [-1,1]}
\label{tab:20x20_3200}
\end{table}


\begin{table}[h]
\centering
\begin{tabular}{@{}llll@{}}
\toprule
Run & \begin{tabular}[c]{@{}l@{}}Total\\ Steps\end{tabular} & \begin{tabular}[c]{@{}l@{}}Predicted\\ Steps\end{tabular} & \begin{tabular}[c]{@{}l@{}}Greedy\\ Steps\end{tabular} \\ \midrule
 1 & 150 & 69 & 81 \\
 2 & 150 & 69 & 81 \\
 3 & 150 & 69 & 81 \\
 4 & 150 & 69 & 81 \\
 \bottomrule
\end{tabular}
\caption{Grid 20x20 with memory size of 4000 items | target (6,18) | reward normalised [-1,1]}
\label{tab:20x20_3200}
\end{table}


\begin{table}[h]
\centering
\begin{tabular}{@{}llll@{}}
\toprule
Run & \begin{tabular}[c]{@{}l@{}}Total\\ Steps\end{tabular} & \begin{tabular}[c]{@{}l@{}}Predicted\\ Steps\end{tabular} & \begin{tabular}[c]{@{}l@{}}Greedy\\ Steps\end{tabular} \\ \midrule
 1 & 500 & 244 & 256 \\
 2 & 500 & 244 & 256 \\
 3 & 500 & 244 & 256 \\
 4 & 500 & 244 & 256 \\
 \bottomrule
\end{tabular}
\caption{Grid 40x40 with memory size of 1600 items | target (6,18)}
\label{tab:20x20_3200}
\end{table}

\subsubsection{Single target}
Here we evaluate the network robustness and ability to improve navigation over multiple flights to a single target position.







\begin{table}[h]
\begin{tabular}{@{}lllllll@{}}
\toprule
\multicolumn{1}{|l|}{\multirow{2}{*}{Approach}} & \multicolumn{1}{l|}{\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Grid\\ Size\end{tabular}}} & \multicolumn{2}{c|}{Training}                                                                              & \multicolumn{3}{c}{Testing}                                                                        \\ \cmidrule(l){3-7} 
\multicolumn{1}{|l|}{}                          & \multicolumn{1}{l|}{}                                                                     & \multicolumn{1}{c|}{Time} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Target\\ Location\end{tabular}} & \multicolumn{1}{c|}{Target Location} & \multicolumn{1}{c|}{Steps} & \multicolumn{1}{c|}{Obstacles} \\ \midrule
Q-learning                                      & 10x10                                                                                     &                           &                                                                                &                                      &                            &                                \\
Guided Q-learning                               & 10x10                                                                                     &                           &                                                                                &                                      &                            &                                \\
MT Q-learning                                   & 10x10                                                                                     &                           &                                                                                &                                      &                            &                                \\
Q-learning                                      & 20x20                                                                                     &                           &                                                                                &                                      &                            &                                \\
Guided Q-learning                               & 20x20                                                                                     &                           &                                                                                &                                      &                            &                                \\
MT Q-learning                                   & 20x20                                                                                     &                           &                                                                                &                                      &                            &                                \\ \bottomrule
\end{tabular}
\end{table}



\subsubsection{Multiple target positions}
The following set of results evaluates the network's robustness and efficiency during single flight mission with multiple target location.

\subsection{Mapping}
\subsubsection{Single Target}

\subsubsection{Multiple Target Positions}

\subsection{Generalisation to Unseen Domains}


\begin{table}[]
\caption{Overall performance under varying weather conditions.}
\resizebox{\columnwidth}{!}{
\label{tab:ddrn_ours}
\begin{tabular}{@{}clllll@{}}
\toprule
Test & Approach & Steps (avg) & Reward (avg) & Completed & Time \\ \midrule
\multirow{2}{*}{III} & $\mathbf{{DRQN^*}_{100}}$ & \textbf{7.35} & \textbf{0.6315} & 118 & \textbf{26.38 minutes} \\
 & Our Approach & 7.5 & 0.4162 & 125  & 29.63 minutes \\ \midrule
\multirow{2}{*}{IV} & ${DRQN^*}_{100}$  & 8.2 & 0.4452 & 124 & 29.48 minutes \\
 &  \textbf{Our Approach}  & \textbf{7.45} & \textbf{0.4883} & 116 & \textbf{26.44 minutes} \\ \midrule
\multirow{2}{*}{V} & ${DRQN^*}_{100}$ & 8.8 & 0.2573 & 129 & 32.73 minutes \\ 
 & \textbf{Our Approach} & \textbf{7.5} & \textbf{0.5079} & 131 & \textbf{30.46 minutes} \\ \midrule
\multirow{2}{*}{VI} & ${DRQN^*}_{100}$ & 9.25 & 0.1642 & 110 & 28.21 minutes \\
 & \textbf{Our Approach} & \textbf{7.48} & \textbf{0.4617} & 132 & 30.96 minutes \\ \midrule
\multirow{2}{*}{VII} & ${DRQN^*}_{100}$ & 7.41 & 0.6467 & 129 & 29.55 minutes \\
 & \textbf{Our Approach} & \textbf{7.23} & \textbf{0.5224} & \textbf{109} & \textbf{23.85 minutes} \\ \midrule
\multirow{2}{*}{VIII} & ${DRQN^*}_{100}$ & 8.03 & 0.4875 & 148 & 35.64 minutes \\
 & \textbf{Our Approach} & \textbf{7.36} & \textbf{0.5365} & \textbf{132} & \textbf{29.95 minutes} \\  
 \bottomrule
\end{tabular}
}
\end{table}

==> root.tex <==
\input{lib/packages.tex}
%\addbibresource{bibliography.bib}

\begin{document}
ghgj

    % \input{tex/0.front-matter.tex}
    % \input{tex/1.introduction.tex}
    % \input{tex/2.related-work.tex}
    % \input{tex/3.methodology.tex}
    % \input{tex/4.experimental-setup.tex}
    % \input{tex/5.results.tex}
    % \input{tex/6.conclusion.tex}
      % \input{tex/7.references.tex}
      \bibliographystyle{IEEEtran}
\bibliography{bibliography.bib}
    %\listoftodos

     
%\printbibliography
\end{document}

